Evidence of large scale energy cascade in the spiral galaxy NGC 5236

Turbulence plays an important role in the structure and dynamics of the galaxy and influences various processes therein including star formation. In this work, we investigate the large scale turbulence properties of the external spiral galaxy NGC 5236. We combine the VLA multi-configuration archival data with the new GMRT observation to estimate the column density and line of sight velocity fluctuation power spectra for this galaxy over almost two decades of length scales. The energy input scale to the ISM turbulence is found to be around $6$ kpc. Power spectra of the two-dimensional turbulence in the galaxy's disk follow a power law with a slope $-1.23\pm0.06$ for the column density and $-1.91\pm0.08$ for the line of sight velocity. The measured power spectra slopes strongly suggest in favour of a compressive forcing with a steady energy input of $\sim 7 \times 10^{-11}$ erg cm$^{-2}$ sec$^{-1}$. We conclude that much of these originate from the gravitational instabilities and self-gravity in the disk. This is the first and most comprehensive study of turbulence statistics for any external spiral galaxy.

==> Tab1.tex <==
\begingroup
\begin{table}
	
\setlength{\tabcolsep}{1pt} % Default value: 6pt
\renewcommand{\arraystretch}{.8}
\begin{tabular}{|c|c|c|c|c|}
\hline
  &
$P_{HI}(\vec{U})$ & $P_{HI}(\vec{U})$ &
$P_{HI}(\vec{U})$ &
$P_{v}(\vec{U})$\\ \hline \hline
Telescope & VLA & GMRT & Combined & GMRT \\  \hline 
$A (\times 10^{4}) $                  & $4.0 \pm 0.8$ & $5.0 \pm 0.6$ & $4.0 \pm 0.4 $ & $88 \pm  9 ^{*}$ \\ \hline
$\alpha$             & $-1.2 \pm 0.3 $             & $-1.24 \pm 0.07$              & $-1.23 \pm 0.06$               & $-1.91 \pm 0.08$ \\ \hline
reduced $\chi^2$ & 1.7& 1.1& 1.1& 1.1\\ \hline
$U_{min} (K\lambda) $& 0.6                          & 0.9                          & 0.4                          & 0.9             \\ \hline
$U_{max} (K\lambda) $& 3                          & 16                         & 16                         & 16            \\ \hline
$R_{min} (Kpc)$      & 1.4                          & 0.3                          & 0.3                           & 0.3             \\ \hline
$R_{max} (Kpc)  $    & 9                          & 5                         & 11                          & 6            \\ \hline
\label{tab:tab1}
\end{tabular}
\caption{Result of power law fit ($P = A U^{\alpha}$) to the column density ($P_{\rm HI}$) and velocity ($ P_v$) power spectra. The power law amplitude ($A$) at one steradian, best fit slope $\alpha$, $1-\sigma$ errors associated with the fit, the reduced $\chi^2$ values and the range of fit in baselines and corresponding length scale ranges are shown. The density power spectra fit are shown for the THINGS VLA data, the GMRT data and the combined power spectra. The velocity power spectra results are only from the GMRT data. The amplitudes for the density spectra are scaled by a factor of $10^4$ and have a unit of steradian. $^*$The amplitude of the velocity spectra are not scaled and is given in (km sec$^{-1}$) $^2$ steradian. }
\end{table}
\endgroup



==> Tab2.tex <==
\begingroup
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{.8} % Default value: 1
\begin{table}
\begin{tabular}{|lccc|}
\hline
Type of \\ Turbulence   & $P_{\rm HI}(\vec{U})$  & $P_{v}(\vec{U})$  & References  \\ \hline \hline
Kolmogorov  		& -                   & $-5/3$            & \citet{1941DoSSR..30..301K}\\ 
Burger's    		& -                   & $-2$              & \citet{BURGERS1948171}\\
	Weizsacker              & $6\alpha - 1$       & $-5/3 - 2\alpha$  & \citet{1996ApJ...458..739F} \\
Solenoidal  		& $-0.78\pm0.06$      & $-1.86\pm0.05$    & \citet{2009ApJ...692..364F}\\ 
Compressive 		& $-1.44\pm0.23$      & $-1.94\pm0.05$    & \citet{2009ApJ...692..364F}\\ 
NGC~5236		& $-1.23\pm0.06$      & $-1.91\pm0.08$    &  This work\\ \hline
\end{tabular}
\caption{Power spectral slope for density and velocity for different theoretical models of turbulence and simulations. All the spectral slopes are given for what is expected for turbulence in the thin disk as the case for this observational result.}
\label{tab:comp}
\end{table}
\endgroup

